Advances in Symmetry Breaking for SAT Modulo Theories

Symmetry breaking is a popular technique to reduce the search space for SAT solving by exploiting the underlying symmetry over variables and clauses in a formula. The key idea is to first identify sets of assignments which fall in the same symmetry class, and then impose ordering constraints, called Symmetry Breaking Predicates (SBPs), such that only one (or a small subset) of these assignments is allowed to be a solution of the original SAT formula. While this technique has been exploited extensively in the SAT literature, there is little work on using symmetry breaking for SAT Modulo Theories (SMT). In SMT, logical constraints in SAT theories are combined with another set of theory operations defined over non-Boolean variables such as integers, reals, etc. SMT solvers typically use a combination of SAT solving techniques augmented with calls to the theory solver. In this work, we take up the advances in SAT symmetry breaking and apply them to the domain of SMT. Our key technical contribution is the formulation of symmetry breaking over the Boolean skeleton variables, which are placeholders for actual theory operations in SMT solving. These SBPs are then applied over the SAT solving part of the SMT solver. We implement our SBP ideas on top of CVC4, which is a state-of-the-art SMT solver. Our approach can result in significantly faster solutions on several benchmark problems compared to the state-of-the-art. Our final solver is a hybrid of the original CVC4 solver, and an SBP based solver, and can solve up to 3.8% and 3.1% more problems in the QF_NIA category of 2018 and 2019 SMT benchmarks, respectively, compared to CVC4, the top performer in this category.

==> theory.tex <==
\section{Theory}
\label{sect:theory}
Before we go to formal description of how we add SBPs in an SMT formulation, let us get some intuition. Existing literature on SBPs already tells us how to exploit symmetries over purely logical formulas. Further, the tool psySMT extends the symmetries over Boolean formulas to the case variables in an SMT formula. 


At the outset, it is not clear how to exploit these symmetries (and SBPs constructed over them) for SMT formulas. One possible approach, as taken by PySMT~\cite{}, is to directly compute symmetries over the SMT formula and construct SBPs corresponding to them. 
In this section, we present our framework for definig SBPs for an SMT theory. 
Let $\Omega$ be an SMT theory which can be written as $\Omega=\Psi \wedge \Phi$ where $\Omega$ is the Boolean skeleton for $\Omega$. Then, we proceed in the following steps.

We formally define the procedure, theory and the proof of the key technical innovation in this section.

Suppose there exists a SMT problem $\Omega$ over a theory $T$ and variable set $V$. Let $A$ be an assignment over the variable set which is defined as a mapping of each variable in the problem to some value in the domain of the theory to which the variable belongs. Le the model set be $M$ which is the set of all the satisfying assignments of that problem. 

Most of the modern day SMT solvers yices \cite{yices}, veriT\cite{verit}, cvc4 \cite{cvc4}
form a Boolean skeleton $\Psi$ by replacing the theory operations by (new) Boolean variables, while enforcing the consistency constraints given by $\Phi$.
Note that the technique discussed here can be applied to any SMT solver that follows this method. Also, it is easy to see that problem formed by $\Psi$ $\land$ $\Phi$ is equivalent to the original problem $\Omega$. All the assignments that satisfy $\Omega$ also satisfies the problem $\Psi$ $\land$ $\Phi$ and vice versa. Here, the values for Boolean skeleton variables is constructed from the constraint set. This allows us to apply symmetry techniques on the problem $\Psi$ $\land$ $\Phi$ instead of original problem $\Omega$.

\begin{algorithm}[]
\SetAlgoLined
\KwResult{Model $M$ for $\Omega$ or UNSAT} 
 $\Psi \leftarrow $ Boolean-Skeleton ($\Omega$);\\
 $\Phi \leftarrow$ Constraint-Set($\Omega$);\\
 $V \leftarrow$ Variable-Ordering;\\
 $\theta_1,\theta_2\cdots\theta_n \leftarrow$ Symmetry-Permutations($\Psi \land \Phi$);\\
 \For{$i\gets0$ \KwTo $n$ }{
    $\mathcal{T} \leftarrow$ SBP-Form($\theta_i, V$);\\
    $\Psi \leftarrow \Psi \land \mathcal{T}$ ;\\   
  }
 $A \leftarrow $ SAT-Solve ($\Psi$);\\
 \While{$\Psi$ is SAT}{
  \eIf{T-consistent($\Phi, A$)}{
   $M \leftarrow$ T-Model($\Phi$)\;
   return $M$\;
   }{
    $C \leftarrow$ Conflict-Clause($\Phi, A$);\\
    $\Psi \leftarrow \Psi \land C$ ;\\
    $A \leftarrow $ SAT-Solve ($\Psi$);\\
  }
 }
 return UNSAT\;\\
 \caption{SMT solving algorithm + Symmetry Breaking Technique}
\end{algorithm}

Now, let us define a permutation $\theta$ over variables set $V$. Application of the permutation on SMT problem $\Omega$ means that for every variable, replacing $v$ with $\theta$(v) in the problem. Let $M$' be the model set for the new problem $\theta$($\Omega$) and $A$' be the assignments in the model $M$'. It is easy to see that 

$A$' $\in$ $M$' iff [$\forall$ $v$ $\in$ $V$, $A$'($\theta$($v$)) = $A$($v$) ] and $A$ $\in$ $M$, 

A symmetry permutation is that permutation which when applied to the problem results in the same problem. This means that simple syntactic reordering of the variables over the ordering invariant operators in the permuted problem results in the original problem. Let $\theta$ be the symmetry permutation of $\Psi$ $\land$ $\Phi$. This means the model set $M$ of the original problem and the set $M$' of the permuted problem are the same. This also means that for every satisfying assignment $A$ of the problem there exists another assignment $A$' such that $\forall$ $v$ $\in$ $V$,  $A$'($\theta$($v$)) = $A$($v$) where $\theta$ is the symmetry. 

The goal of the symmetry breaking technique is to add a predicate such that only the lexicographically smaller assignment (under a given variable ordering) between $A$ and $A$' is chosen resulting in pruning of the search space. Since we are only interested in the satisfiability of the problem, there is no harm in adding a constraint that one of the assignments out $A$ and $A$' satisfy. Such a constraint is called Symmetry Breaking Predicate or simply SBP. 

This is achieved by adding a predicate of the form: 
\begin{equation}
\wedge_{1 \le i \le n} (\wedge_{1 \le j < i} v_j = \theta(v_j)) \Rightarrow v_i \Rightarrow \theta(v_i)
\end{equation}
It is known as SBP~\cite{crawford}. Here, $n$ is the total number of variables, and $v_1,v_2\cdots,v_n$ is the variable ordering. It is now easy to prove that at least one of the $A$ and $A$' satisfies the above SBP formulation. If we arrange the assignments $A$ and $A$' based on a variable ordering then, the SBP simply says that only lexicographically smaller one will be satisfied.  
\begin{theorem}
The SMT problem represented by $\Psi \land \Phi$ and $(\Psi  \land \mathcal{T}) \land \Phi$ are equi-satisfiable where the notations are as defined in Algorithm 2
\end{theorem}

Since we find the symmetry $\theta$ over the problem $\Psi$ $\land$ $\Phi$, we restrict ourselves to symmetries in which at least one Boolean skeleton variable is permuted to another skeleton variable. Most of the SMT solvers iterate over the satisfying truth assignments of the boolean skeleton $\Psi$ while checking the theory consistency at each step. Therefore, by adding SBP restricted to only boolean skeleton variables directly to the skeleton structure $\Psi$, help us restrict the number of such satisfying assignments. Note that the symmetry $\theta$ captures the syntactic information of both theory variables and the boolean skeleton variables in itself and addition of such restricted SBP allows us to exploit this information effectively.

Also, the technique seems to be particularly helpful in case of UNSAT problems. To prove any problem UNSAT, the solver has to search the entire space of truth assignments and each of the try results in a failure. Pruning some of the space seems to guarantee improvement in performance. However, for the SAT problems, adding SBPs can be both boon and bane depending on the problem. If the assignment we prune, was a valid solution then we unnecessarily reject it and search further. In other case, we achieve speed-up by pruning an unnecessary path. We address this issue using ensemble methods discussed in the sub-section below. Further, it can also be easily inferred that our method is more successful in those categories of problems in which the underlying theory is very complex. This is a direct result of the fact that we prune assignments in the boolean space and if solver had explored those paths then it would have cost an overhead equal to time required for checking the theory consistency of the assignment. This time would be much more for theories like Non-Linear over Linear and Integer over Reals. This hypothesis was confirmed in our experiments. 


%We add the following two major extensions to the basic algorithm described above by the CVC4 solver.
\subsection{Symmetry Breaking Technique}
\begin{table*}[t]
\centering
\caption{Symmetry Breaking Technique}\smallskip
\begin{tabular}{ll}
SMT Problem  $\Omega$                       & $((z > 2) \lor (x < 8)) \land ((z > 2) \lor (y < 8)) \land ((x+y < 10) \lor (x+y > 3)) $                                               \\
Boolean Skeleton  $\Psi$                    & $(P \lor Q) \land (P \lor R) \land (S \lor T)$                                                                           \\
Constraints Set  $\Phi$                     & $(P \Leftrightarrow (z > 2)) \land (Q \Leftrightarrow (x < 8)) \land (R \Leftrightarrow (y < 8)) \land (S \Leftrightarrow (x + y < 10)) \land (T \Leftrightarrow (x + y > 3))$ \\
Satisfying Assignment &  $z=3; x=7; y=9; P=True; Q=True; R=False; S=False; T=True$ \\
Symmetry Permut.  $\theta$                 & $\theta(Q) = R$;  $\theta(R) = Q$; $\theta(x) = y; \theta(y) = x$                                                   \\
Satisfying Assignment & $ z=3; x=9; y=7; P=True; Q=False; R=True; S=False; T=True $\\
SBP added $\mathcal{T}$                                  & $Q \Rightarrow R$                                                                                       \\
New Skeleton $\Psi$ $'$ & $(P \lor Q) \land (P \lor R) \land (S \lor T) \land (\neg Q \lor R)$ \\
Assignment chosen & $ z=3; x=9; y=7; P=True; Q=False; R=True; S=False; T=True $
\end{tabular}
\label{table1}
\end{table*}



%Such a formulation helps us to add symmetries over both theory 
 % results   the variables in $\Psi$ and $\Phi$ results in identical formulation for the skeleton as well as the constraint set. %Note that this results in identical SMT formulation.
% Then, it is straightforward to show that if $M$ is a model (satisfying assignment) of the SMT problem then $\theta(M)$ is also a model $\theta$ being a symmetry. 
% Further, the theory of symmetry breaking ensures that only the lexicographically smaller model (under a given variable ordering) between $M$ and $\theta(M)$ is chosen resulting in pruning of the search space. 

%is done by adding what is referred to as an SBP, i.e., a symmetry breaking predicate. from the theory of symmetry breaking~\cite{crawfard}, (1) if $M$ is a model then $\theta(M)$ is also a model, and (2) given a variable ordering, we can choose lexicographically smaller model by adding an SBP enforcing only one of $\theta(M) $ and $M$ is chosen for all models $M$. This results in SBP given by $\mathcal{T}$ in the above example (under the variable ordering $Q < R < S < T$). Application of this SBP preserves satisifiability of the resulting SMT problem. 
%The key innovation here is the application of
%our ability to apply 
%these SBPs over the Boolean skeleton variables (only) while ensuring the corresponding symmetries hold for the variables in the skeleton as well as the constraint set. This results in  a sound formulation preserving the satisfiability. 
%the skeleton variables as well as those in the constraint set resulting in a sound formulation. % resulting in a sound formulation.
%resulting in a sound formulation.  
The table 1 provides an example with a  problem with linear integer theory. 
The SBP ($\mathcal{T}$) in the example above is $Q\Rightarrow R$, under the variable ordering $P,Q,R,S,T$. The $A'$ assignment is selected over $A$ and hence the solver do not have to explore both of them. 
%also hold satisfied over the constraint set. 
%simultaneously over the Boolean skeleton as well as the constraint set. 

In order to maximize the impact of SBPs formed and reduce overheads we introduce various heuristics explained in the subsections below.  
% We have designed some heuristics in choosing the variable ordering in order to maximize the impact of SBPs formed. Further, we restrict the size of the SBP formed to reduce overhead as done by earlier work~\cite{aloul}.

%careful in choosing the variable ordering that maximises the impact of the SBPs formed. We also restrict the size of the SBPs formed to reduce the overheads \cite{aloul}.
%of the form given by $$$M \rightarrow \theta(M)$ resulting in SBP of the form .

%add an SBP () to eliminate the 
%Consider the above SMT problem $\Omega$, the boolean skeleton $\Psi$ is being formed by assigning the propositional variables to each of the constraints $\Phi$. As we can see, $\Psi$ and $\Phi$ together form the same problem as $\Omega$. We then use SyMT tool to find the symmetry permutation $\Pi$ for this problem. Symmetry permutation is defined as a map from variable to variable, which when applied to the SMT problem, leaves the problem unchanged. The presence of such a permutation suggests that if there exists a model M that satisfies the original problem, then there will always exist another model M\textsc{\char13} with permutation applied to the model M. Therefore, if a variable ordering is defined, we can choose the lexicographically smaller model out of M and M\textsc{\char13} by adding the Symmetry Breaking Predicate without changing the satisfiability of the problem. The SBP is added to the original boolean skeleton $\Psi$ to form a new skeleton $\Psi$\textsc{\char13} which will have a smaller search space than the original one. Since we have to try lesser number of truth assignments to the boolean variables, we are able to find a solution earlier. We have also been careful in choosing the variable ordering that maximises the impact of the SBPs formed. We also restrict the size of the SBPs formed to reduce the overheads \cite{aloul}. 
% \vspace{-0.1in}
\subsection{Variable Ordering Heuristic}
The step in line 3 of algorithm 2 mentions about choosing a variable ordering to define lexicographic relation between solutions. The symmetry breaking technique is invariant of any arbitrary variable ordering chosen. Also, once the ordering is chosen, it must remain consistent for all the symmetries detected. However, to maximize the effect of the process, we tried different heuristics on the variable ordering. The key idea here is to make the new clause added to play a significant role in deciding the truth assignment for the boolean skeleton. We choose the variables appearing as positive unit variables in the clausal normal form of the boolean skeleton to appear first in the variable ordering. The main intuition behind such a choice lies the fact that most SAT solvers first assign true values to these unit variables for unit propagation, and hence for the Symmetry Breaking Predicate of the form $v \Rightarrow \theta(v)$ , the value of $\theta(v)$ gets automatically decided. The SAT solver will now directly assign $True$ value to the $\theta(v)$ and hence pruning the branch where it could have been assigned a $False$. This simple heuristic boosts the performance of the technique discussed here.

\subsection{Reduced Size Heuristic}
The step mentioned in line 6 of the Algorithm 2 involve forming SBP from the found symmetry permutation. Although we mention the general form of SBP added in the theory section, but we are free to choose any subset of that SBP without breaking the soundness. As suggested by \cite{shatter} in the Symmetry Breaking for SAT solving, breaking all symmetries may not speed up the search because there are often exponentially many of them and may be redundant. We restrict to single symmetry generators given by graph-automorphism solver of \cite{symt}. Further, it was seen that smaller generator cycles seems to be more effective. Therefore, we restrict the size of permutations larger than k bits to k, where k is a hyperparameter.   
\subsection{Ensemble Technique}
We in our experiments found that there are a lot of non-overlapping problems solved by algorithm 1 and Algorithm 2 in the SMT benchmarks. Particularly, for the 2018 QF\_NIA benchmarks, we saw that algorithm 2 is able to solve large number of benchmarks that algorithm 1 was not able to solve. However, there was another equally large chunk of problems in which algorithm 1 beat algorithm 2. Hence, the overall gain in the number of benchmarks solved was quite low. This means that for several problems adding SBPs resulted in significant speed-ups, whereas in other cases, it slowed down the original solver. We hypothesize this is because in the former case, unnecessary parts of the search space are pruned resulting in speed-up, whereas in the latter case, the SBPs might be pruning valid models, resulting in further delay in reaching a satisfying assignment. 

Taking insight from this, we design an ensemble solver, where we first run the solver with SBPs added for a fixed time $t$, and if the solution is still not found, we resort to the original solver with SBPs removed. $t$ is a hyperparameter. %of the model. 
This results in significant boost in performance compared to CVC4 on a subset of SMT benchmarks. %number of benchmark problems.
%approach results in best of both worlds, and we can solve a significantly large number of problems compared to CVC4 on a subset of benchmark categories.
%before timing out in some of the categories.
%our solver can be significantly faster the base solver CVC4 on a number of benchmark problems.
%, and our solver can solve a significantly large number of problems in a subset of categoriesour approach can solve close to $700$ additional problems compared to the base CVC4 solver in the NIA cateogry of $\cite{$ resulting a solving a large fraction of benchmark problems in the SMT-COMP~\cite{SMT-COMT-18} 
%On experimenting with the symmetry breaking technique for the SMT solvers, we found that in some problems, it helps to reduce time taken by the solver significantly while in others, it in-fact increases the time used. This behaviour could be explained by the fact that sometimes, pruning the search-space rejects a model that might have been found early-on in the search path, while sometimes it helps to find a solution early by cutting out parts in the search tree which could have been searched unnecessarily before reaching to that solution. To get the best of both the worlds, we ran CVC4 with SBPs for some fixed portion of time in the time-limit and then restarted with the original CVC4 without the additional clauses. This helps to significantly boost the performance.  
%------------------------------------------------------------------------------
